Strategic Plan for a Scientific Software Innovation Institute (S2I2) for High Energy Physics

The quest to understand the fundamental building blocks of nature and their interactions is one of the oldest and most ambitious of human scientific endeavors. Facilities such as CERN's Large Hadron Collider (LHC) represent a huge step forward in this quest. The discovery of the Higgs boson, the observation of exceedingly rare decays of B mesons, and stringent constraints on many viable theories of physics beyond the Standard Model (SM) demonstrate the great scientific value of the LHC physics program. The next phase of this global scientific project will be the High-Luminosity LHC (HL-LHC) which will collect data starting circa 2026 and continue into the 2030's. The primary science goal is to search for physics beyond the SM and, should it be discovered, to study its details and implications. During the HL-LHC era, the ATLAS and CMS experiments will record circa 10 times as much data from 100 times as many collisions as in LHC Run 1. The NSF and the DOE are planning large investments in detector upgrades so the HL-LHC can operate in this high-rate environment. A commensurate investment in R&D for the software for acquiring, managing, processing and analyzing HL-LHC data will be critical to maximize the return-on-investment in the upgraded accelerator and detectors. The strategic plan presented in this report is the result of a conceptualization process carried out to explore how a potential Scientific Software Innovation Institute (S2I2) for High Energy Physics (HEP) can play a key role in meeting HL-LHC challenges.

==> questions-focus-areas.tex <==

\begin{enumerate}

\item {\bf Impact - Physics:} Will efforts in this area enable new approaches to computing and software that maximize, and could potentially radically extend, the physics reach of the detectors?
\item {\bf Impact - Resources:} Will efforts in this area achieve required improvements in software efficiency, scalability and performance and make use of the advances in CPU, storage and network technologies?
\item {\bf Impact - Sustainability:} Will efforts in this area guarantee the long term sustainability of the software through the lifetime of the HL-LHC?
\item {\bf Interest/Expertise:} Does the U.S.\ university community have a strong interest and expertise in the area?
\item {\bf Leadership:} Are the proposed focus areas complementary to efforts funded by the US-LHC Ops programs, DOE or international entities?
\item {\bf Value:} Is there potential to provide value to more than one LHC experiment and to the wider HEP community?
\item {\bf Research/Innovation:} Are there opportunities for combining research and innovation as part of partnerships between the HEP and Computer Science communities?
%\item Does the area offer opportunities for integration of cutting-edge training and education for our students and postdocs?
\end{enumerate}




==> workshop-participants-by-workshop.tex <==
\noindent{\s2i2-HEP workshop at ACAT:}
\vskip 0.1in
Peter Elmer (Princeton University),
Mike Sokoloff (University of Cincinnati),
Mark Neubauer (University of Illinois at Urbana-Champaign),
Miron Livny (University of Wisconsin - Madison),
Brian Bockelman (University of Nebraska - Lincoln),
Ruslan Mashinistov (University of Texas at Arlington),
Jeff Carver (University of Alabama),
Horst Severini (University of Oklahoma),
Justas Balcas (Caltech),
Ilija Vukotic (University of Chicago),
Dan Katz (University of Illinois at Urbana-Champaign),
Jim Pivarski (Princeton University),
Sergei Gleyzer (University of Florida),
Karen Tomko (Ohio Supercomputer Center),
Michela Paganini (Yale University),
Amir Farbin (University of Texas at Arlington),
Tanu Malik (Depaul University),
Elizabeth Sexton-Kennedy (FNAL),
David Lange (Princeton University),
Carlos Maltzahn (University of California - Santa Cruz),
Henry Schreiner (University of Cincinnati),
Oliver Gutsche (FNAL),
Kaushik De (University of Texas at Arlington),
Mike Hildreth (Notre Dame),
Daniel Elvira (FNAL),
Bo Jayatilaka (FNAL),
Lothar Bauerdick (FNAL),
Rob Kutschke (FNAL),
Gordon Watts (University of Washington),
Jim Kowalkowski (FNAL),
Dan Riley (Cornell University),
Jerome Lauret (BNL),
Antonio Augusto Alves Junior (University of Cincinnati),
Frank Wuerthwein (UCSD),
Charlotte Lee (University of Washington),
Sudhir Malik (University of Puerto Rico),
Maria Girone (CERN),
Wahid Bhimji (NERSC/LBNL),
Kyle Cranmer (NYU),
Justin Wozniak (ANL),

\vskip 0.2in
\noindent{HSF Workshop in Annecy:}
\vskip 0.1in

Frederique Chollet (LAPP),
Peter Elmer (Princeton University),
David Lange (Princeton University),
Dan Katz (University of Illinois at Urbana-Champaign),
Daniel Elvira (FNAL),
Oliver Gutsche (FNAL),
Jim Pivarski (Princeton University),
Matt Bellis (Siena College),
Bo Jayatilaka (FNAL),
Torre Wenaus (BNL),
Frank Wuerthwein (UCSD),
Kaushik De (UT Arlington),
Cecile Barbier (LAPP),
Nadine Neyroud (LAPP),
Jean Jacquemier (LAPP),
Thomas Vuillaume (LAPP),
Valentin Kuznetsov (Cornell University),
Sebastien Binet (IN2P3/LPC),
Hadrien Grasland (Universite de Paris-Sud),
Oliver Keeble (CERN),
Dario Menasce (INFN Milano),
Michel Jouvin (LAL/Universite de Paris-Sud),
Helge Meinhard (CERN),
Sergei Gleyzer (University of Florida),
Shawn McKee (University of Michigan),
John Harvey (CERN),
Ian Collier (RAL),
Paolo Calafiura (LBNL),
Ian Bird (CERN),
Pere Mato (CERN),
Elizabeth Sexton-Kennedy (FNAL),
Graeme Stewart (University of Glasgow),
Mark Neubauer (Univ. Illinois at Urbana-Champaign),
Dirk Duellmann (CERN),
Eduardo Rodrigues (University of Cincinnati),
Maria Girone (CERN),
Andrea Valassi (CERN),
Patricia Mendez Lorenzo (CERN),
Vassil Vassilev (Princeton University),
Michael Sokoloff (University of Cincinnati),
Markus Schulz (CERN),
Stefan Roiser (CERN),
Ken Bloom (University of Nebraska-Lincoln),
Makoto Asai (SLAC),
Gordon Watts (U.Washington),
Mike Hildreth (Notre Dame),
Ian Fisk (Simons Foundation),
Rob Kutschke (FNAL),
Markus Klute (MIT),
Jean-Roch Vlimant (Caltech),
Michael Kirby (FNAL),
Patrick Skubic (University of Oklahoma),
Antonio Augusto Alves Junior (University of Cincinnati),
Marc Verderi (Ecole Polytechnique),
Sabine Elles (LAPP),
Matthew Feickert (Southern Methodist University),
Meghan Kane (Soundcloud, MIT)),
David Rousseau (LAL-Orsay),
Rob Gardner (University of Chicago),
Peter Onyisi (University of Texas at Austin),
Simone Campana (CERN),
Lothar Bauerdick (FNAL),
Harvey Newman (Caltech),
Giulio Eulisse (CERN),
Paul Laycock (CERN),
Giacomo Govi (FNAL),
Amir Farbin (UT Arlington),
Vladimir Gligorov (CNRS),
Eric Lancon (BNL),
Benedikt Hegner (CERN),
Martin Ritter (LMU Munich),
Tommaso Boccali (INFN Pisa),
Daniele Bonacorsi (INFN Bologna),
Benjamin Couturier (CERN),
Richard Mount (SLAC),
Thomas McCauley (Notre Dame),
Fernanda Psihas (U.Indiana),
Riccardo Bianchi (U.Pittsburg),
Gloria Corti (CERN),
Lukas Heinrich (NYU),
Pierre Aubert (LAPP),
Andrei Gheata (CERN),
Catherine Biscarat (CNRS),
Farah Hariri (CERN),
Jamie Bedard (Siena College),
Madeline Hagen (Siena College),
Conor Fitzpatrick (EPFL),
John Apostolakis (CERN),
Tom Gibbs (NVIDIA),
Johannes Albrecht (TU Dortmund),


\vskip 0.2in
\noindent{CWP Frameworks Workshop at FNAL:}
\vskip 0.1in

Chris Green (FNAL),
Benedikt Hegner (CERN),
Kyle Knoepfel (FNAL),
Jim Kowalkowski (FNAL),
Thomas Kuhr (LMU),
Charles Leggett (LBNL),
Adam Lyon (FNAL),
David Malon (Argonne National Laboratory),
Marc Paterno (FNAL),
Elizabeth Sexton-Kennedy (FNAL),
Vakho Tsulaia (LBNL),

\vskip 0.2in
\noindent{HEP Analysis Ecosystem Retreat in Amsterdam:}
\vskip 0.1in

David Smith (CERN),
Dirk Duellmann (CERN),
Mike Sokoloff (U.Cincinnati),
Peter Elmer (Princeton University),
Jim Pivarski (Princeton University),
Eduardo Rodrigues (U.Cincinnati),
Axel Naumann (CERN),
Fons Rademakers (CERN),
Federico Carminati (CERN),
Dario Menasce (INFN Milano),
Brian Bockelman (U.Nebraska-Lincoln),
Gordon Watts (U.Washington),
Graeme Stewart (U.Glasgow),
Pere Mato (CERN),
Lukasz Kreczko (Bristol),
Attila Krasznahorkay (CERN),
Oliver Gutsche (FNAL),
Liz Sexton-Kennedy (FNAL),
Philippe Canal (FNAL),
Enric Tejedor Saavedra (CERN),
Vassil Vassilev (Princeton University),
Torre Wenaus (BNL),
Paul Laycock (CERN),
Roger Jones (Lancaster),
Gerardo Ganis (CERN),
Sebastian Binet (Universite de Paris-Sud),
David Lange (Princeton University),
Markus Schulz (CERN),
Andrea Rizzi (INFN-Pisa),
Benedikt Hegner (CERN),
Marcin Nowak (CERN),
Frank Wuerthwein (UCSD),
Peter Hristov (CERN),
Jeff Templon (Nikhef),
Maria Girone (CERN),
Andrew Gilbert (KIT),
Martin Ritter (LMU Munich),
Vincent Croft (Nikhef),
Antonio Augusto Alves Jr (U.Cincinnati),
Patrick Bos (Netherlands eScience Center),
Mark Neubauer (U.Illinois at Urbana-Champaign),
Anton Poluektov (University of Warwick),
Wouter Verkerke (Nikhef),
Chris Tunnell (U.Chicago),
Giulio Eulisse (CERN),
Gerhard Raven (Nikhef),
Gianluca Cerminara (CERN),
Sascha Caron (Nikhef),
Steven Schramm (Universite de Geneve),
Jakob Blomer (CERN),
Kyle Cranmer (New York University),
Max Baak (KPMG),
Kurt Rinnert (U.Liverpool),
Simone Campana (CERN),
Meghan Kane (SoundCloud, MIT),


\vskip 0.2in
\noindent{\s2i2-HEP/CS workshop at Princeton:}
\vskip 0.1in

Peter Elmer (Princeton University),
Michael Sokoloff (University of Cincinnati),
Daniel S. Katz (University of Illinois Urbana-Champaign),
Mark Neubauer (University of Illinois at Urbana-Champaign),
Jim Pivarski (Princeton University),
Shawn McKee (University of Michigan),
Oliver Gutsche (Fermi National Accelerator Laboratory),
Rob Gardner (University of Chicago),
Miron Livny (University of Wisconsin-Madison),
Shantenu Jha (Rutgers/Brookhaven),
Carlos Maltzahn (University of California, Santa Cruz),
Elizabeth Sexton-Kennedy (Fermilab),
Lawrence R Frank (UCSD),
Ilija Vukotic (University of Chicago),
Eric Vaandering (Fermilab),
Lothar Bauerdick (Fermilab),
Michela Taufer (University of Delaware),
Charlotte Lee (University of Washington),
Christopher Jones (Fermi National Accelerator Laboratory),
Matthew Bellis (Siena College/Cornell University),
Paolo Calafiura (LBNL),
Matthew Feickert (Southern Methodist University),
Manish Parashar (Rutgers University),
Kaushik De (University of Texas at Arlington),
Jeffrey Carver (University of Alabama),
Sergei Gleyzer (University of Florida),
Harvey Newman (Caltech),
Tanu Malik (DePaul University),
Mike Hildreth (University of Notre Dame),
Matthieu Lefebvre (Princeton University),
Ian Cosden (Princeton University),
Robert Knight (Princeton University),
Doug Benjamin (Duke University),
Douglas Thain (University of Notre Dame),
Sudhir Malik (University of Puerto Rico Mayaguez),
Nan Niu (University of Cincinnati),
Justin M Wozniak (Argonne National Laboratory),
Meghan Frate (University of California, Irvine),
Valentin Kuznetsov (Cornell University),
Frank Wuerthwein (UCSD/SDSC),
Sunita Chandrasekaran (University of Delaware),
Gabriel Perdue (Fermilab),
Anton Burtsev (University of California, Irvine),
Adam Aurisano (University of Cincinnati),
Spencer Smith (McMaster University),
Fernanda Psihas (Indiana University),
Kyle Cranmer (NYU),
Michael Kirby (Fermilab),
Kyle Knoepfel (Fermi National Accelerator Laboratory),
Robert Illingworth (Fermilab),
Gordon Watts (University of Washington),
Rick Wagner (Globus),
Isobel Ojalvo (Princeton University),
Lukas Heinrich (New York University),
Dustin Tran (Columbia University),
Michael Andrews (Carnegie Mellon University/CERN),
Chris Tunnell (UChicago, KICP),
Rajesh Ranganath (Princeton University),
Meghan Kane (SoundCloud, MIT) ,
Patrick de Perio (Columbia University),
Vinod Gupta (Princeton University),
Joon Kim (Princeton University),
Karan Bhatia (Google Cloud),
Alexey Svyatkovskiy (Princeton University),
Sumit Saluja (Princeton University),

\vskip 0.2in
\noindent{HSF workshop at UCSD/SDSC:}
\vskip 0.1in

David Abdurachmanov (University of Nebraska-Lincoln),
Mohammad Al-Turany (GSI),
Johannes Albrecht (TU Dortmund),
Dustin Anderson (California Institute of Technology),
Makoto Asai (SLAC National Accelerator Laboratory),
Justas Balcas (Caltech),
Lothar Bauerdick (Fermilab),
Dario Berzano (CERN),
Wahid Bhimji (Berkeley Lab),
Riccardo Maria Bianchi (University of Pittsburgh),
Ian Bird (CERN),
Brian Bockelman (University of Nebraska-Lincoln),
Amber Boehnlein (Jefferson Lab),
Daniele Bonacorsi (University of Bologna),
Joseph Boudreau (University of Pittsburgh),
Paolo Calafiura (LBNL),
Simone Campana (CERN),
Louis Capps (NVIDIA),
Federico Carminati (CERN),
Taylor Childers (Argonne Nat. Lab),
Kaushik De (Univ. of Texas at Arlington),
Andrea Dotti (SLAC National Accelerator Laboratory),
Peter Elmer (Princeton University),
V. Daniel Elvira (Fermilab),
Giulio Eulisse (CERN),
Amir Farbin (University of Texas Arlington),
Ian Fisk (Simons Foundation),
Frank Gaede (DESY),
Rob Gardner (University of Chicago),
Maria Girone (CERN),
Sergei Gleyzer (University of Florida),
Vladimir Gligorov (CNRS),
Claudio Grandi (INFN),
Lindsey Gray (Fermilab),
Dick Greenwood (Louisiana Tech University),
Oliver Gutsche (Fermi National Accelerator Laboratory),
Thomas Hacker (Purdue University),
Andrew Hanushevsky (SLAC National Accelerator Laboratiry),
John Harvey (CERN),
Richard Hay Jr (Princeton University),
Benedikt Hegner (CERN),
Lukas Heinrich (New York University),
Mike Hildreth (Notre Dame),
Burt Holzman (Fermilab),
Dirk Hufnagel (Fermilab),
Bo Jayatilaka (Fermilab),
Shantenu Jha (Rutgers University),
Ivo Jimenez UC (Santa Cruz),
Christopher Jones Fermi National Accelerator Laboratory),
Michel Jouvin CNRS/LAL),
Daniel S. Katz (University of Illinois),
Dorian Kcira (California Institute of Technology),
Alexei Klimentov (Brookhaven National Lab),
Thorsten Kollegger (GSI),
Jim Kowalkowski (Fermilab),
Slava Krutelyov (UC San Diego),
Robert Kutschke (Fermilab),
Valentin Kuznetsov (Cornell University),
Eric Lancon (BNL),
David Lange (Princeton University),
Kevin Lannon (University of Notre Dame),
Mario Lassnig (CERN),
Matthieu Lefebvre (Princeton University),
Antonio Limosani (CERN / University of Sydney),
Miron Livny (University of Wisconsin-Madison),
Carlos Maltzahn (University of California, Santa Cruz),
Aashrita Mangu (California Institute of Technology),
Pere Mato (CERN),
Paul Mattione (Jefferson Lab),
Thomas McCauley (University of Notre Dame),
Helge Meinhard (CERN),
Dario Menasce (INFN Milano-Bicocca),
Parag Mhashilkar (Fermilab),
Bogdan Mihaila (NSF),
Lorenzo Moneta (CERN),
Richard Mount (SLAC),
Alja Mrak Tadel (Univerity California San Diego),
Mark Neubauer (University of Illinois at Urbana-Champaign),
Harvey Newman (Caltech),
Bill Nitzberg (Altair),
Nan Niu (University of Cincinnati),
Peter Onyisi (University of Texas at Austin),
Jim Pivarski (Princeton University),
Rob Quick (Indiana University),
Nathalie Rauschmayr (CERN),
Stefan Roiser (CERN),
Paul Rossman (Google Inc.),
David ROUSSEAU (LAL-Orsay),
Aaron Sauers (Fermilab),
Markus Schulz (CERN),
Ariel Schwartzman (SLAC),
Horst Severini (University of Oklahoma),
Michael Sevilla (University of California, Santa Cruz),
Elizabeth Sexton-Kennedy (Fermilab),
Michael Sokoloff (University of Cincinnati),
Maria Spiropulu (Caltech),
Graeme Stewart (University of Glasgow),
Ian Stockdale (Altair Engineering),
Matevz Tadel (UCSD),
Anyes Taffard (UC Irvine),
Giacomo Tenaglia (CERN),
Karen Tomko (Ohio Supercomputer Center),
Konstantin Toms (University of New Mexico),
Vakho Tsulaia (LBNL),
Eric Vaandering (Fermi National Accelerator Laboratory),
Andrea Valassi (CERN),
Jean-Roch Vlimant (California Institute of Technology),
Ilija Vukotic (University of Chicago),
Noah Watkins (University of California, Santa Cruz),
Torre Wenaus (BNL),
Sandro Wenzel (CERN),
Daniel Whiteson (UC Irvine),
Nancy Wilkins-Diehr (University of California San Diego),
Mike Williams (MIT),
Justin Wozniak (University of Chicago),
Wenjing Wu (Institute of High Energy Physics),
Frank Wuerthwein (UCSD/SDSC),
Avi Yagil (UCSD),
Graham Mackintosh (IBM),
Jeff Hammond (Intel),






\vskip 0.2in
\noindent{\s2i2-HEP/CS workshop at UIUC:}
\vskip 0.1in
D. Adrovic (DePaul), 
Adam Aurisano (Cincinnati), 
Lothar Bauerdick (FNAL), 
Paolo Calafiura (LBNL), 
Jeffrey Carver (Alabama), 
K. Chard (Chicago), 
Kaushik De (Texas, Arlington), 
A. Elliott (Aegis Research Labs), 
Peter Elmer (Princeton), 
Neil Ernst (Software Engineering Institute), 
Amir Farbin (Texas, Arlington), 
Matthew Feickert (Southern Methodist), 
Rob Gardner (Chicago), 
Sandra Gesing (Notre Dame), 
Sergei Gleyzer (Florida), 
D. Greenwood (Louisiana Tech), 
Thomas Hacker (Purdue), 
Ben Hooberman (Illinois), 
K. Huff (Illinois), 
Shantenu Jha (Rutgers), 
R. Kalescky (Southern Methodist), 
Dan Katz (Illinois/NCSA), 
Jim Kowalkowski (FNAL), 
A. Kumar (Southern Methodist), 
David Lange (Princeton), 
D. Lesny (Illinois), 
Miron Livny (Wisconsin), 
Carlos Maltzahn (Santa Cruz), 
S. Mannam (DePaul), 
Ajit Majumder (Wayne State), 
Shawn McKee (Michigan), 
Mark Neubauer (Illinois), 
Nan Niu (Cincinnati), 
Peter Onyisi (Texas), 
Don Petravick (Illinois/NCSA), 
Marc Paterno (FNAL), 
Jim Pivarski (Princeton), 
Jeff Porter (LBNL), 
B. Riedel (Chicago), 
Henry Schreiner III (Cincinnati), 
Sally Seidel (New Mexico), 
Elizabeth Sexton-Kennedy (FNAL), 
Mike Sokoloff (Cincinnati), 
Doug Thain (Notre Dame), 
M.Turk (Illinois), 
John Towns (Illinois/NCSA), 
Iljia Vukotic (Chicago), 
Justin Wozniak (ANL), 
Frank Wuerthwein (San Diego),
M. Zhang (Illinois),



